Formalization of Phase Ordering

Phasers pose an interesting synchronization mechanism that generalizes many collective synchronization patterns seen in parallel programming languages, including barriers, clocks, and point-to-point synchronization using latches or semaphores. This work characterizes scheduling constraints on phaser operations, by relating the execution state of two tasks that operate on the same phaser. We propose a formalization of Habanero phasers, May-Happen-In-Parallel, and Happens-Before relations for phaser operations, and show that these relations conform with the semantics. Our formalization and proofs are fully mechanized using the Coq proof assistant, and are available online.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{D. Orchard and N. Yoshida (Eds.): Programming Language Approaches to \\ Concurrency- and Communication-Centric Software (PLACES 2016).\\
EPTCS 211, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.211.2}{10.4204/EPTCS.211.2}}
\pdfoutput=1

